Exploiting Strict Constraints in the Cylindrical Algebraic Covering

One of the few available complete methods for checking the satisfiability of sets of polynomial constraints over the reals is the cylindrical algebraic covering (CAlC) method. In this paper, we propose an extension for this method to exploit the strictness of input constraints for reducing the computational effort. We illustrate the concepts on a multidimensional example and provide experimental results to evaluate the usefulness of our proposed extension.

==> acm.tex <==
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10002950.10003705.10003707</concept_id>
       <concept_desc>Mathematics of computing~Solvers</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10003752.10003790.10003794</concept_id>
       <concept_desc>Theory of computation~Automated reasoning</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010148.10010149.10010150</concept_id>
       <concept_desc>Computing methodologies~Algebraic algorithms</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Mathematics of computing~Solvers}
\ccsdesc[500]{Theory of computation~Automated reasoning}
\ccsdesc[500]{Computing methodologies~Algebraic algorithms}

